Wide & Deep Learning for Judging Student Performance in Online One-on-one Math Classes

In this paper, we investigate the opportunities of automating the judgment process in online one-on-one math classes. We build a Wide & Deep framework to learn fine-grained predictive representations from a limited amount of noisy classroom conversation data that perform better student judgments. We conducted experiments on the task of predicting students' levels of mastery of example questions and the results demonstrate the superiority and availability of our model in terms of various evaluation metrics.

==> related.tex <==
Judging students' classroom performance is assumed to be a necessary condition for adaptive classroom instructions and various studies and approaches have been proposed along this direction \cite{freeman1993two,begeny2008teachers,sudkamp2012accuracy,praetorius2013judgment,praetorius2017identifying,praetorius2015judging,sturmer2013declarative}. Existing research about teacher judgment can be categorized into two categories: measuring the accuracy of teacher judgments, and improving teacher judgment accuracy.

% \vspace{-0.4cm}
\subsection{Measuring the accuracy of teacher judgments}
% \vspace{-0.1cm}

The most common approach used to measure judgment accuracy is computing the correlation between teachers' predictions of students' performance and students' actual academic performance \cite{freeman1993two,begeny2008teachers,sudkamp2012accuracy,praetorius2013judgment}. For examples, Freeman studied the results of predictions made by 13 elementary school teachers of 214 students' achievement in Grades 4 to 6 on the Gates-MacGinitie Reading Test \cite{freeman1993two}. Begeny et al. examined relationship between the teacher's perceptions of students' reading abilities and students' oral reading fluency performance across a continuum of rating methods \cite{begeny2008teachers}. S{\"u}dkamp et al. conducted a meta-analysis research  and described multiple factors constitute judgment accuracy, such as teacher and student characteristics \cite{sudkamp2012accuracy}. Furthermore, Praetorius et al. examined how confident teachers are in their judgments of students' mathematics and verbal self-concepts, and whether judgment confidence is related to judgment accuracy \cite{praetorius2013judgment}. 

% \vspace{-0.4cm}
\subsection{Improving teacher judgment accuracy}
% \vspace{-0.1cm}

Various research studies focus on making teaching more effective by improving the accuracy of teachers' judgments \cite{praetorius2015judging,sturmer2013declarative,sahebi2018student,dhamecha2018balancing}. Praetorius et al. conducted a zero-acquaintance study to demonstrate the possibility of accurately judging students' self-concept based on 30-second videos of students \cite{praetorius2015judging}. S{\"u}dkamp et al. studied the process of developing the judgment ability as a knowledge-guided process and shown that effective teaching of video-based course will help teachers gain knowledge in student performance prediction  \cite{sturmer2013declarative}. Dhamecha et al.  developed an iterative data collection and grading approach to improve the student response analysis task in dialog-based intelligent tutoring systems \cite{dhamecha2018balancing}. Recently, researchers start to investigate to use eye-tracking or gaze-tracking tools to improve teachers' ability to assess student characteristics \cite{mcintyre2019capturing,sturmer2013declarative,haataja2019teacher}. McIntyre et al. analyzed teachers' gaze proportions to study their different expertise related and cultural priorities \cite{mcintyre2019capturing}. Haataja et al. explored the relations between teachers' scaffolding intentions and their gaze behaviors \cite{haataja2019teacher}. Besides, there are several research works focusing on teacher judgment specifically in programming classes such as identifying tinkering behaviors and finding struggling students when doing programming assignments \cite{dong2021using,gao2021early}. 

% and furthermore, \cite{haataja2021relation} expanded the study to understand the teacher-student eye contacts in relation to teachers' interpersonal behavior

Our work is different from aforementioned methods since both of them try to manually conduct user studies to verify the accuracy of teacher judgment and the corresponding effects and influence. Meanwhile, the majority of existing works in above approaches use the results of assignments or exams to represent student performance, which is a very lagged and coarse indicator. In our work, we use the state-of-the-art neural network approaches to automatically judge student performance by analyzing the teacher-student in-class conversational ASR transcriptions in a much more fine-grained level. Please note that our work is distinguished from (1) dropout prediction in the massive open online courses because there is no instructors conducting live teaching in MOOCs \cite{tang2018time} and (2) item response theory and knowledge tracing since we focus on prediction with rich in-class teacher-student interaction data instead of the sequential correct or incorrect responses of problems solved by the students \cite{embretson2013item,corbett1994knowledge,piech2015deep}.



